Identifying dark matter interactions in monojet searches

We study the discrimination of quark-initiated jets from gluon-initiated jets in monojet searches for dark matter using the technique of averaged jet energy profiles. We demonstrate our results in the context of effective field theories of dark matter interactions with quarks and gluons, but our methods apply more generally to a wide class of models. Different effective theories of dark matter and the standard model backgrounds each have a characteristic quark/gluon fraction for the leading jet. When used in conjunction with the traditional cut-and-count monojet search, the jet energy profile can be used to set stronger bounds on contact interactions of dark matter. In the event of a discovery of a monojet excess at the 14 TeV LHC, contact interactions between dark matter with quarks or with gluons can be differentiated at the 95% confidence level. For a given rate at the LHC, signal predictions at direct detection experiments for different dark matter interactions can span five orders of magnitude. The ability to identify these interactions allows us to make a tighter connection between LHC searches and direct detection experiments.

==> searches_old.tex <==
In this section we discuss the EFT approach to study DM contact interactions with quarks and gluons. We will summarize the current limits placed on the scale of the contact interactions by monojet searches at the LHC.

\subsection{The effective field theory approach}
The EFT approach to DM at the LHC was first studied
in~\cite{Goodman:2010yf,Goodman:2010ku,Bai:2010hh,Rajaraman:2011wf,Fox:2011pm}.
We will briefly recap the approach from these papers. We will consider
Dirac fermion DM with contact operators of dimension 6 and 7 that
couple pairs of dark matter particles to SM light quarks and gluons
respectively.


\blue{get rid of this, introduce the operators we are considering directly, then discuss the ones we are not considering}
The operators are of the form:
\begin{align}
  \mathcal{O}_\textrm{dim 6} = \frac{1}{M^2_*} (\bar{q}  \Gamma q)( \bar{\chi} \Gamma_\chi \chi), \\
  \mathcal{O}_\textrm{dim 7} = \frac{\alpha_s}{M^3_*} (G  \Gamma' G) (\bar{\chi} \Gamma_\chi' \chi),
\end{align}
where the $\Gamma$, $\Gamma'$ are different matrices needed to
construct appropriate Lorentz covariant bilinears.\red{Does the gluon
operator ever have/need a matrix?} For quark contact operators, the
scalar quark bilinears $(\bar{q}_L q_R)$, $(\bar{q}_R q_L)$ are
expected to be suppressed by the light quark masses and so we will not
consider them. The vector $(\bar{q} \gamma_\mu q)$ and axial vector
$(\bar{q} \gamma_\mu \gamma_5 q)$ operators give practically similar
limits at collider searches, but the difference is important when we
consider direct detection experiments because the former gives rise to
spin independent interactions with nuclei, which are strongly
constrained, whereas the latter give spin dependent interactions,
which are weakly constrained. \blue{For this collider study we will
therefore only consider the vector bilinear operator for quarks.}
\textbf{need to discuss what to do about spin dependent.}

For simplicity, we will will focus on just two operators,
\begin{align}
\Oq = \frac{1}{M^2_*} (\bar{q}  \gamma_\mu q)( \bar{\chi} \gamma^\mu \chi), \\
\Og = \frac{\alpha_s}{4 M^3_*} (G^a_{\mu\nu} G^{a\mu\nu}) (\bar{\chi} \chi).
\end{align}
Here, the normalization has been chosen in accord with
Ref.~\cite{Goodman:2010ku}, where $\mathcal{O}_q$ and $\mathcal{O}_g$
are referred to as D5 and D11 in their study. For each choice of
operator we have a simplified model to study at the LHC, with only two
parameters: the dark matter mass, $\MDM$ \red{mass=$m_\chi$?} and the
cutoff scale, $M_*$.

\subsection{Searches and limits at the LHC}
The effective operator formalism is useful for defining simplified
model parameters for DM that can be tested at the LHC. The operators
$\Oq$ and $\Og$, combined with ISR, can give rise to monojet
signatures defined as a high energy jet accompanied by large $\MET$ at
the LHC. The most dominant SM background comes from $Z + j$ with $Z
\rightarrow \nu \bar{\nu}$, there are sub-dominant backgrounds from $W
+ j$ with $W \rightarrow \tau \nu$,  where the $\tau$ decays
hadronically and $W \rightarrow \mu \nu$ or $e \nu$, where the lepton
is misidentified as a jet. \red{We should differentiate between
irreducible and reducible backgrounds. Also mention that for JEP the Q
and Z look the same, so a scaled Zj suffices}.
\blue{After imposing the cuts, the $Z + j$
background is typically a factor of a few larger than all the other
backgrounds combined. In our study we will hence focus only on the
$Z+j$ background.}\red{Details of the background modeling are given
in section \ref{subsec:bkg_methods} }.


In order to discover an excess in monojets a \textsl{cut-and-count}
strategy is used by the ATLAS and CMS experiments
\cite{ATLAS-CONF-2012-147, CMS-PAS-EXO-12-048}. \textbf{For low values
of the dark matter mass}, the $\MET$ or $p_T$ spectrum of the monojet
associated with DM production is more slowly falling relative to the
$p_T$ of the background. By choosing different values of the $p_T$ and
$\MET$ cut, the experimentalists \red{the analysis defines} are able to define different ``signal
regions'' (SR) in which they try to place limits on the suppression
scale, $M_*$ for a given value of $\MDM$ \red{again}. Choosing too low
a value of
the $p_T$ and $\MET$ cuts leads to the errors on the background events
being dominated by systematics, whereas too high a value of the $p_T$
cut reduces the number of events on which to perform statistical
analysis.

We will adopt the so-called SR3 region from the ATLAS searches
\red{signular?}, which
they use to set limits on the scale $M_*$. In this region, the
statistical errors are comparable to the systematic errors.

The following cuts are required for event selection in this region:
\begin{itemize}
\item $\MET > 350$~GeV,
\item leading jet with $p_T > 350$~GeV and $|\eta| < 2.0$,
\item at most two jets with $p_T > 30$~GeV and $|\eta| < 4.5$,
\item $\Delta \phi$ (jet, $\MET$) $> 0.5$ (second leading jet),
\item lepton vetoes. \red{any lepton vetoed? should we discuss how our
  lepton veto might be more effective, since we never fail to
  reconstruct the lepton?}
\end{itemize}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
%  \includegraphics[width=7.5cm,height=7.5cm,keepaspectratio]{qqchichi_explimit}
   \psfragfig*[width=7.5cm,keepaspectratio]{qqchichi_explimit}{
  \psfrag{X}[c][t][0.8]{\mvu{-0.2}{$m_\chi$ (GeV)}}
  \psfrag{Y}[c][b][0.8]{\mvu{0.3}{$M_*$ (GeV)}}
  \psfrag{Q}{\mvl{4}{$ \Oq = \frac{1}{M^2_*} (\bar{q}  \gamma_\mu q)( \bar{\chi} \gamma^\mu \chi) $}}
  \psfrag{A}{\mvl{5.5}{ATLAS 90\% CL exclusion}}
  \psfrag{C}{\mvl{5.5}{CMS 95\% CL exclusion}}
  \psfrag{1000}{\mvl{0.2}{$ 1000 $}}
  \psfrag{900}{\mvl{0.2}{$ 900 $}}
  \psfrag{800}{\mvl{0.2}{$ 800 $}}
  \psfrag{700}{\mvl{0.2}{$ 700 $}}
  \psfrag{600}{\mvl{0.2}{$ 600 $}}
  \psfrag{500}{\mvl{0.2}{$ 500 $}}
  \psfrag{400}{\mvl{0.2}{$ 400 $}}
  \psfrag{350}{\mvl{0.2}{$ 350 $}}
  \psfrag{300}{\mvl{0.2}{$ 300 $}}
  \psfrag{250}{\mvl{0.2}{$ 250 $}}
  \psfrag{200}{\mvl{0.2}{$ 200 $}}
  \psfrag{150}{\mvl{0.2}{$ 150 $}}
  \psfrag{100}{\mvl{0.2}{$ 100 $}}
  \psfrag{50}{\mvl{0.2}{$ 50 $}}
  \psfrag{20}{\mvl{0.2}{$ 20 $}}
  \psfrag{10}{\mvl{0.2}{$ 10 $}}
  }
  \caption{Limit on $M_*$ from $O_q$.}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
 % \includegraphics[width=7.5cm,height=7.5cm,keepaspectratio]{ggchichi_explimit}
     \psfragfig*[width=7.5cm,keepaspectratio]{ggchichi_explimit}{
  \psfrag{X}[c][t][0.8]{\mvu{-0.2}{$m_\chi$ (GeV)}}
  \psfrag{Y}[c][b][0.8]{\mvu{1.0}{$M_*$ (GeV)}}
  \psfrag{G}{\mvu{0.25}{\mvl{5}{$ \Og = \frac{\alpha_s}{4 M^3_*} (G^a_{\mu\nu} G^{a\mu\nu}) (\bar{\chi} \chi) $}}}
  \psfrag{A}{\mvl{4}{ATLAS 90\% CL exclusion}}
  \psfrag{C}{\mvl{4}{CMS 95\% CL exclusion}}
  \psfrag{1000}{\mvl{0.2}{$ 1000 $}}
  \psfrag{900}{\mvl{0.2}{$ 900 $}}
  \psfrag{800}{\mvl{0.2}{$ 800 $}}
  \psfrag{700}{\mvl{0.2}{$ 700 $}}
  \psfrag{600}{\mvl{0.2}{$ 600 $}}
  \psfrag{500}{\mvl{0.2}{$ 500 $}}
  \psfrag{400}{\mvl{0.2}{$ 400 $}}
  \psfrag{350}{\mvl{0.2}{$ 350 $}}
  \psfrag{300}{\mvl{0.2}{$ 300 $}}
  \psfrag{250}{\mvl{0.2}{$ 250 $}}
  \psfrag{200}{\mvl{0.2}{$ 200 $}}
  \psfrag{150}{\mvl{0.2}{$ 150 $}}
  \psfrag{100}{\mvl{0.2}{$ 100 $}}
  \psfrag{50}{\mvl{0.2}{$ 50 $}}
  \psfrag{20}{\mvl{0.2}{$ 20 $}}
  \psfrag{10}{\mvl{0.2}{$ 10 $}}
  }
  \caption{Limit on $M_*$ from $O_g$.}
  \label{fig:sub2}
\end{subfigure}
\caption{ATLAS \cite{ATLAS-CONF-2012-147} and CMS \cite{CMS-PAS-EXO-12-048} exclusions on the suppression scale $M_*$ for various dark matter masses from the 8 TeV run of the LHC. ATLAS used 10.5~fb$^{-1}$ of luminosity for their analysis, whereas CMS used 19.5~fb$^{-1}$ of luminosity. CMS has not yet released an official limit for the $O_g$ operator.}
\label{fig:explimits}
\end{figure}

The resulting limits in the $\MDM - M_*$ plane from non-observation of an excess in monojets at the 8~TeV run of the LHC are shown for the operators $\Oq$ and $\Og$ in Fig.~\ref{fig:explimits}. Strictly speaking, the validity of the effective theory description restricts the values of $\sqrt{s} \lesssim M_*$, where $s$ is the square of the typical center-of-mass energy of the initial partons. However, even for regions where the effective theory is invalid, the experimental bounds in the $\MDM - M_*$ plane can give a qualitative understanding of the bounds on dark matter physics models.

To gain an understanding of the typical kinematics of the monojet signal, we plot the expected event distribution as a function of the invariant mass of the DM particles ($m_{\bar{\chi}\chi}$) and the jet $p_T$ in Fig.~\ref{fig:kinematics}. Practically of course, only the jet $p_T$ of the events is observable, however, this plot is instructive because we can see that the typical center of mass energy, $s \simeq m^2_{\bar{\chi}\chi} + p^2_T$, \blue{is much larger than the current bounds on the effective theory scale $M_*$. Nevertheless, we will continue to use the EFT description and it will not affect our main conclusions.}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
%  \includegraphics[width=7.cm,height=7.0cm,keepaspectratio]{qqchichi_mchichivspt}
       \psfragfig*[width=7.5cm,keepaspectratio]{qqchichi_mchichivspt}{
   \psfrag{X}[c][t][0.8]{\mvu{-0.2}{jet $p_T$ (GeV)}}
  \psfrag{Y}[c][b][0.8]{\mvu{1.2}{$m_{\bar{\chi}\chi}$ (GeV)}}
  \psfrag{G}{\mvu{0.25}{\mvl{4}{$ \Og = \frac{\alpha_s}{4 M^3_*} (G^a_{\mu\nu} G^{a\mu\nu}) (\bar{\chi} \chi) $}}}
  \psfrag{A}{\mvl{4}{ATLAS 90\% CL exclusion}}
  \psfrag{C}{\mvl{4}{CMS 95\% CL exclusion}}
  \psfrag{2000}{\mvl{0.4}{$ 2000 $}}
  \psfrag{1500}{\mvl{0.4}{$ 1500 $}}
  \psfrag{1000}{\mvl{0.4}{$ 1000 $}}
  \psfrag{900}{\mvl{0.2}{$ 900 $}}
  \psfrag{800}{\mvl{0.2}{$ 800 $}}
  \psfrag{700}{\mvl{0.2}{$ 700 $}}
  \psfrag{600}{\mvl{0.2}{$ 600 $}}
  \psfrag{500}{\mvl{0.4}{$ 500 $}}
  \psfrag{400}{\mvl{0.2}{$ 400 $}}
  \psfrag{350}{\mvl{0.2}{$ 350 $}}
  \psfrag{300}{\mvl{0.2}{$ 300 $}}
  \psfrag{250}{\mvl{0.2}{$ 250 $}}
  \psfrag{200}{\mvl{0.2}{$ 200 $}}
  \psfrag{440}{\mvl{0.2}{$ 440 $}}
  \psfrag{420}{\mvl{0.2}{$ 420 $}}
  \psfrag{380}{\mvl{0.2}{$ 380 $}}
  \psfrag{360}{\mvl{0.2}{$ 360 $}}
  \psfrag{0}{\mvl{0.4}{$ 0 $}}
  \psfrag{1.}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 1. $}}}}
  \psfrag{0.9}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.9 $}}}}
  \psfrag{0.8}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.8 $}}}}
  \psfrag{0.7}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.7 $}}}}
  \psfrag{0.6}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.6 $}}}}
  \psfrag{0.5}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.5 $}}}}
  \psfrag{0.4}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.4 $}}}}
  \psfrag{0.3}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.3 $}}}}
  \psfrag{0.2}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.2 $}}}}
  }
  \caption{Event kinematic distribution for the $\Oq$ operator.}
  \label{fig:sub3}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
 % \includegraphics[width=7.cm,height=7.0cm,keepaspectratio]{ggchichi_mchichivspt}
       \psfragfig*[width=7.5cm,keepaspectratio]{ggchichi_mchichivspt}{
  \psfrag{X}[c][t][0.8]{\mvu{-0.2}{jet $p_T$ (GeV)}}
  \psfrag{Y}[c][b][0.8]{\mvu{1.2}{$m_{\bar{\chi}\chi}$ (GeV)}}
  \psfrag{G}{\mvu{0.25}{\mvl{4}{$ \Og = \frac{\alpha_s}{4 M^3_*} (G^a_{\mu\nu} G^{a\mu\nu}) (\bar{\chi} \chi) $}}}
  \psfrag{A}{\mvl{4}{ATLAS 90\% CL exclusion}}
  \psfrag{C}{\mvl{4}{CMS 95\% CL exclusion}}
   \psfrag{2000}{\mvl{0.4}{$ 2000 $}}
    \psfrag{1500}{\mvl{0.4}{$ 1500 $}}
  \psfrag{1000}{\mvl{0.4}{$ 1000 $}}
  \psfrag{900}{\mvl{0.2}{$ 900 $}}
  \psfrag{800}{\mvl{0.2}{$ 800 $}}
  \psfrag{700}{\mvl{0.2}{$ 700 $}}
  \psfrag{600}{\mvl{0.2}{$ 600 $}}
  \psfrag{500}{\mvl{0.4}{$ 500 $}}
  \psfrag{400}{\mvl{0.2}{$ 400 $}}
  \psfrag{350}{\mvl{0.2}{$ 350 $}}
  \psfrag{300}{\mvl{0.2}{$ 300 $}}
  \psfrag{250}{\mvl{0.2}{$ 250 $}}
  \psfrag{200}{\mvl{0.2}{$ 200 $}}
  \psfrag{150}{\mvl{0.2}{$ 150 $}}
  \psfrag{100}{\mvl{0.2}{$ 100 $}}
  \psfrag{50}{\mvl{0.2}{$ 50 $}}
  \psfrag{20}{\mvl{0.2}{$ 20 $}}
  \psfrag{10}{\mvl{0.2}{$ 10 $}}
  \psfrag{440}{\mvl{0.2}{$ 440 $}}
  \psfrag{420}{\mvl{0.2}{$ 420 $}}
  \psfrag{380}{\mvl{0.2}{$ 380 $}}
  \psfrag{360}{\mvl{0.2}{$ 360 $}}
  \psfrag{0}{\mvl{0.4}{$ 0 $}}
  \psfrag{1.}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 1. $}}}}
  \psfrag{0.9}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.9 $}}}}
  \psfrag{0.8}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.8 $}}}}
  \psfrag{0.7}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.7 $}}}}
  \psfrag{0.6}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.6 $}}}}
  \psfrag{0.5}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.5 $}}}}
  \psfrag{0.4}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.4 $}}}}
  \psfrag{0.3}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.3 $}}}}
  \psfrag{0.2}{\mvu{-0.3}{\mvl{-0.4}{\tiny{$ 0.2 $}}}}
  }
  \caption{Event kinematic distribution for the $\Og$ operator.}
  \label{fig:sub4}
\end{subfigure}
\caption{Plot of the distribution of monojet signal events as a function of invariant mass of the $\bar{\chi}\chi$ and jet $p_T$ in different EFTs. The normalization of the event distribution is arbitrary. \blue{We can see that most events are produced with a large center of mass energy, greater than the current bound on the scale of the effective operators, $M_*$ .}}
\label{fig:kinematics}
\end{figure}

